Disentangling and Operationalizing AI Fairness at LinkedIn

Operationalizing AI fairness at LinkedIn's scale is challenging not only because there are multiple mutually incompatible definitions of fairness but also because determining what is fair depends on the specifics and context of the product where AI is deployed. Moreover, AI practitioners need clarity on what fairness expectations need to be addressed at the AI level. In this paper, we present the evolving AI fairness framework used at LinkedIn to address these three challenges. The framework disentangles AI fairness by separating out equal treatment and equitable product expectations. Rather than imposing a trade-off between these two commonly opposing interpretations of fairness, the framework provides clear guidelines for operationalizing equal AI treatment complemented with a product equity strategy. This paper focuses on the equal AI treatment component of LinkedIn's AI fairness framework, shares the principles that support it, and illustrates their application through a case study. We hope this paper will encourage other big tech companies to join us in sharing their approach to operationalizing AI fairness at scale, so that together we can keep advancing this constantly evolving field.

==> input/aivsequity.tex <==
\section{Equal AI Treatment vs Equitable Outcomes}
\label{sec:aivsequity}

To understand LinkedIn’s approach towards AI Fairness, it is crucial to understand why and how we differentiate between two broad tracks of work, namely Equal AI Treatment and Equitable Outcomes. 

Consider a situation, where we are trying to evaluate the fairness (on binary gender) of a product feature that is recommending connections. This feature is powered by an AI system producing scores for potential connections for each member and shows a fixed-length ranked list to the member, see figure \ref{fig:PYMK}. For more details about the AI model being used in powering this product please see \cite{pymkblog}. In this section, for ease of exposition, let us only focus on fairness with respect to the members being recommended as prospective connections. We expand on the notion of fairness with respect to members viewing these connections in Section \ref{sec:practice}.

Let’s assume that the member $u$ working in an engineering leadership position, receives 5 recommendations in the order M, M, F, M, M, where M represents a male profile and F represents a female. To evaluate fairness, the first intuition is to ensure that the feature is providing equal opportunity for equally qualified members, i.e. the order of the recommendation is in line with their qualification of being a useful professional connection for user $u$ aka “Equal AI Treatment”. One of the simple ways to quantify is through predictive parity \cite{diciccio2022predictive, barocas2017fairness}, i.e., for any given score, the expected qualification of the male demographic is the same as that of the female demographic. We will expand on definitions in Section \ref{sec:practice}. 

Consider in this case that the predictive parity is satisfied, but there is still a lingering large skew in the representation of the male demographic as against female. Despite knowing that the model is ordering the candidates based on qualification, this large skew shows that Equal AI Treatment alone does not address the historical barriers faced by females in getting to engineering leadership positions and hence the skew in the pool of qualified candidates. To address this large skew, strategies might require treating members of various demographics unequally, a concept that must be tackled with utmost care and thoughtfulness to not unintentionally introduce new biases in the system. 

While both Equal AI Treatment and Equitable Outcomes seem necessary, neither of them is sufficient on their own. Moreover, satisfying both of them together may not be possible, unless the underlying qualified population has an almost equal representation. In a problem space that requires more action today than ever before, this conundrum can be quite debilitating for institutions that set out to offer equitable experiences to their members. To help operationalize AI Fairness efforts, the stance LinkedIn has taken is to disentangle the concepts and clearly identify the modus operandi, driver, and platform for each of Equal AI Treatment and Equitable Outcomes as follows: 

\begin{itemize}
\item Equal AI Treatment: AI systems must aim to satisfy “Equal Opportunity for Equally Qualified Members”. 
\item Equitable Outcomes: The solutions must lie in product changes, in the form of UI or policy or net new product features. These changes must be modular, explicit and rooted deeply in understanding the barriers faced by various demographics.
\end{itemize}

